Stranding Risk for Underactuated Vessels in Complex Ocean Currents: Analysis and Controllers

Low-propulsion vessels can take advantage of powerful ocean currents to navigate towards a destination. Recent results demonstrated that vessels can reach their destination with high probability despite forecast errors. However, these results do not consider the critical aspect of safety of such vessels: because of their low propulsion which is much smaller than the magnitude of currents, they might end up in currents that inevitably push them into unsafe areas such as shallow areas, garbage patches, and shipping lanes. In this work, we first investigate the risk of stranding for free-floating vessels in the Northeast Pacific. We find that at least 5.04% would strand within 90 days. Next, we encode the unsafe sets as hard constraints into Hamilton-Jacobi Multi-Time Reachability (HJ-MTR) to synthesize a feedback policy that is equivalent to re-planning at each time step at low computational cost. While applying this policy closed-loop guarantees safe operation when the currents are known, in realistic situations only imperfect forecasts are available. We demonstrate the safety of our approach in such realistic situations empirically with large-scale simulations of a vessel navigating in high-risk regions in the Northeast Pacific. We find that applying our policy closed-loop with daily re-planning on new forecasts can ensure safety with high probability even under forecast errors that exceed the maximal propulsion. Our method significantly improves safety over the baselines and still achieves a timely arrival of the vessel at the destination.

==> xx_lit_review.tex <==
\section{Literature Review}
\label{sec:lit_review}
In this section, we describe the relevant literature spanning 
The related work consists of
\begin{itemize}
    \item Navigating in known flows (A*, RRT, non-linear opt, evolutionary algos). HJ reachability gives time-optimal path
    \item Navigating in unknown flows
    \begin{itemize}
        \item with realistic probability distribution available
        \begin{itemize}
            \item when operating: Monte-Carlo, MDP, Stochastic Reachability
            \item when training/simulating: reinforcement learning
        \end{itemize}
        \item without access to a distribution
        \begin{itemize}
            \item Regular replanning/Receding Horizon Planning (with and without learning about the currents online while operating e.g. with a GP)
            \item Using a control hierarchy (High level planner and low level steering/tracking controller)
            \item Robust control: with Reach-Avoid Games
        \end{itemize}
    \item Closed-loop operation with uncertain dynamics
    \begin{itemize}
        \item Robust MPC Methods
        \item Adaptive control?/Meta learning? (mostly assumes fixed parameters to be learned but for us now information tells us limited amount about the future, it's fundamental epistemic uncertainty)
    \end{itemize}
    \item underactuated control more generally?
    \item where people have used reachability for extracting closed-loop controllers \mwnote{maybe integrate that in method section}
    \begin{itemize}
        \item safety framework
        \item \mwnote{@Claire maybe you know more history on that?}
    \end{itemize}
    \end{itemize}
\end{itemize}

% Computational Complexity of Exact Robust MPC (high, but for us ok)
% Tube based MPC (cite the handbook of MPC by Radovic) /rakovic2018handbook

% as this assumption is quite restrictive when it comes to generating scenarios of heteroscedastic processes, e.g. solar irradiance
% A time series variable is heteroscedastic if the variance changes throughout time.
% Talk about scenario based MPC (which scenario am I in), adaptive MPC (learning about the environment on the go), and stochastic MPC (minimizing an expected cost functional), robust MPC (with dynamic programming we essentially solve the robust MPC problem and it turns out that deterministic MPC performs indeed better than robust as we can see with our data).
